Discriminative Learning of Similarity and Group Equivariant Representations

One of the most fundamental problems in machine learning is to compare examples: Given a pair of objects we want to return a value which indicates degree of (dis)similarity. Similarity is often task specific, and pre-defined distances can perform poorly, leading to work in metric learning. However, being able to learn a similarity-sensitive distance function also presupposes access to a rich, discriminative representation for the objects at hand. In this dissertation we present contributions towards both ends. In the first part of the thesis, assuming good representations for the data, we present a formulation for metric learning that makes a more direct attempt to optimize for the k-NN accuracy as compared to prior work. We also present extensions of this formulation to metric learning for kNN regression, asymmetric similarity learning and discriminative learning of Hamming distance. In the second part, we consider a situation where we are on a limited computational budget i.e. optimizing over a space of possible metrics would be infeasible, but access to a label aware distance metric is still desirable. We present a simple, and computationally inexpensive approach for estimating a well motivated metric that relies only on gradient estimates, discussing theoretical and experimental results. In the final part, we address representational issues, considering group equivariant convolutional neural networks (GCNNs). Equivariance to symmetry transformations is explicitly encoded in GCNNs; a classical CNN being the simplest example. In particular, we present a SO(3)-equivariant neural network architecture for spherical data, that operates entirely in Fourier space, while also providing a formalism for the design of fully Fourier neural networks that are equivariant to the action of any continuous compact group.

==> Chapters/Chapter03/intro.tex <==
\newcommand{\knn}{$k$NN\xspace}

\section{Introduction}
Nearest neighbor methods are among the oldest and the most widely used tools in machine learning. Although nearest neighor rules are often successful, their performance tends to be limited by two factors: the computational cost of searching for nearest neighbors and the choice of the metric (distance measure) defining ``nearest''.  The cost of searching for neighbors can be reduced with efficient indexing,e.g.,~\cite{arya1998optimal,datar2004locality,beygelzimer2006cover} or learning compact representations,e.g.,~\cite{kulis2009learning,wang2010sequential,norouzi2011minimal,gong2011iterative}.  We will not address this issue here.  Here we focus on the choice of the metric. The metric is often taken to be Euclidean, Manhattan or $\chi^2$ distance.  However, it is well known that in many cases these choices are suboptimal in that they do not exploit statistical regularities that can be leveraged from labeled data. This paper focuses on supervised metric learning. In particular, we present a method of learning a metric so as to optimize the accuracy of the resulting nearest neighbor estimator (for classification and regression).

Existing works on metric learning (the overwhelming majority of which is for classification) formulate learning as an optimization task with various constraints driven by considerations of computational feasibility and reasonable, but often vaguely justified principles \cite{Xing02distancemetric,goldberger2004neighbourhood,globersoncollaps06,weinberger2009distance,weinberger2008fast,mcfee10_mlr,kedem2012non,dannytarlowkNCA}.  
A fundamental intuition is shared by most of the work in this area: an ideal distance for prediction is distance in the target space. Of course, that can not be measured, since prediction of a test example's target is what we want to use the similarities to begin with. Instead, one could learn a similarity measure with the goal for it to be a good proxy for the target similarity. Since the performance of $k$NN prediction often is the real motivation for similarity learning, the constraints typically involve ``pulling'' good neighbors (from the correct class for a given point in the case of classification) closer while ``pushing'' the bad
neighbors farther away. The exact formulation of ``good'' and ``bad'' varies but is defined as a combination of proximity and agreement between targets.  We give a formulation that facilitates a more direct attempt to optimize for the $k$NN accuracy as compared to previous work as far as we are aware. We discuss existing methods in more detail in section~\ref{sec:related}, where we also place our work in context. We also show that
our formulation makes it natural to apply standard learning methods for structural latent support vector machines (SVMs) to the problem of supervised metric learning.


\begin{figure*}[!th]\label{fig:LMNNComparison}
  \centering
  \resizebox{.7\textwidth}{!}{\input{./Chapters/Chapter03/lmnnfig}}
  \caption{Illustration of objectives of LMNN (left) and our
    structured approach to ``neighborhood gerrymandering'' (right) for $k=3$. The point $\mathbf{x}$ of
    class blue is the query point. In LMNN, the target points are the
    nearest neighbors of the same class, which are points $a, b$ and
    $c$ (the circle centered at $\mathbf{x}$ has radius equal to th
e farthest of the target points i.e. point b). The LMNN objective will push all the points of the wrong class that lie inside this circle out (points $e, f, h, i, \text{and} j$), while pushing in the target points to enforce the margin. On the other hand, for our structured approach (right), the circle around $\mathbf{x}$ has radius equal to the distance of the farthest of the three nearest neighbors irrespective of class. Our objective only needs to ensure zero loss. This would be achieved by pushing in point $a$ of the correct class (blue) while pushing out the point having the incorrect class (point $f$). Note that two points of the incorrect class lie inside the circle ($e, \text{and} f$), both being of class red. However $f$ is pushed out and not $e$ since it is farther from $\mathbf{x}$. Some more discussion about this is presented in Section \ref{related}.}
\end{figure*}

In the $k$NN prediction problem, given a point and a chosen metric, there is an implicit hidden variable: the choice of $k$ ``neighbors''. The inference of the predicted label from these $k$  examples is trivial: by simple majority vote among the associated labels for classification, and by taking a weighted average in the case of regression. In the case of classification, given a query point, there can possibly exist a very large number of choices of $k$ points that might correspond to zero loss: any set of $k$ points with the majority of correct class will do. Whereas, in the case of regression, there can exist a very large number of choices of $k$ points that might correspond to a loss less than a tolerance parameter (since zero loss would be impossible in most scenarios). We would like a metric to ``prefer'' one of these ``good'' example sets over any set of $k$ neighbors which would vote for a wrong class (or in the case of regression correspond to a high loss). Note that to win, it is not necessary for the right class to account for all the $k$ neighbors -- it just needs to get more votes than any
other class. As the number of classes and the value of $k$ grow, so does the space of available good (and bad) example sets.

These considerations motivate our approach to metric learning. It is akin to the common, albeit negatively viewed, practice of \emph{gerrymandering} in drawing
up borders of election districts so as to provide advantages to desired political parties, e.g., by concentrating voters from that
party or by spreading voters of opposing parties. In our case, the ``districts'' are the cells in the Voronoi diagram defined by the
Mahalanobis metric, the ``parties'' are the class labels voted for by the neighbors falling in each cell, and the ``desired winner'' is the
true label of the training points associated with the cell. This intuition is why we refer to our method as \emph{neighborhood gerrymandering} in the title.


Technically, we write $k$NN prediction as an inference problem with a structured latent variable being the choice of $k$ neighbors. Thus learning involves minimizing a sum of a structural latent hinge loss
and a regularizer \cite{boser1992}. Computing structural latent hinge loss involves loss-adjusted inference --- one must compute loss-adjusted values of both the output value (the label) and the latent items (the set of nearest neighbors). The loss augmented inference corresponds to a choice of worst $k$ neighbors in the sense that while having a high average similarity they also correspond to a high loss (``worst offending set of $k$ neighbors''). Given the inherent combinatorial considerations, the key to such a model is efficient inference and loss augmented inference. We give an efficient algorithm for {\em exact} inference. We also design an optimization algorithm based on stochastic gradient descent on the surrogate loss. Our approach achieves $k$NN accuracy higher than state of the art for most of the data sets we tested on, including some methods specialized for the relevant input domains.

Although we initially restrict ourselves to learning a Mahalanobis distance in an explicit feature space, the formulation is then extended to nonlinear similarity measures such as those defined by nonlinear kernels, provided computing the gradients of similarities with respect to metric parameters is feasible. In this extension, the inference and loss augmented inference steps remain unchanged. Our formulation can also naturally handle a user-defined loss matrix on labels rather than just a zero-one loss. We then also extend the framework to $k$NN regression, which as we describe is intractable in a sense, given that in the case of regression the number of ``classes'' is uncountable. This is attacked by both modifying the objective suitably and presenting algorithms for inference and loss augmented inference tailored for regression. 

\begin{comment}

Nearest neighbor classifiers are among the oldest and the most widely
used tools in machine learning. They are often successful in practice,
but even bigger success has been hampered by two factors. One is the
computational cost of the search for neighbors, especially in high
dimensional feature spaces. Much work has been devoted to alleviating
this difficulty by means of efficient indexing, e.g.,~\cite{arya1998optimal,datar2004locality,beygelzimer2006cover} or learning
compact representations, e.g.,~\cite{kulis2009learning,wang2010sequential,norouzi2011minimal,gong2011iterative}. However, this does not address the
second issue: definition of neighbors as
training instances with minimal distance to the test point relies on a
metric, often Euclidean, Manhattan or $\chi^2$ distance. 
An implicit assumption in this is that the feature space in which the examples
are represented is appropriate for such a comparison. However, it is well known
that in many cases this turns out to be a suboptimal choice of
similarity measure. This motivates the problem of learning a metric (or more generally a distance
measure) from data with the goal of improving classification accuracy
of nearest neighbor methods. Our work belongs in this category of
supervised metric learning.

A fundamental intuition is shared by most of the work in this area: an ideal
distance for prediction is ditance in the label space.
Of course, that can not be measured, since prediction of a test example's label is what we want to
use the similarities to begin with. Instead, one could learn a
similarity measure with the goal for it to be a good proxy for the
label similarity. 

Much of existing work approaches this as an
optimization task with various constraints driven by
considerations of computational feasibility and reasonable, but often
vaguely justified principles. Since the performance of $k$NN
prediction often is the real motivation for similarity learning, the
constraints typically involve ``pulling'' good neighbors (from the
correct class for a given point) closer while ``pushing'' the bad
neighbors farther. However, as far as we are aware, none of previous
work attempts to directly optimize this $k$NN accuracy. This paper
describes our proposal to rectify this situation.

We write the $k$NN prediction as an inference
problem in a structured model, with a latent variable representing the
choice of $k$ neighbors. The key to such a model is efficient
inference, in particular loss augmented inference inherent in
structured learning. We propose an efficient algorithm for
\emph{exact} inference, and design an optimization algorithm based on
stochastic subgradient descent on the surrogate loss, which is a
kind of structured hinge loss.
This allows us to learn similarity
that achieves $k$NN accuracy higher than state of the art for most of
the data sets we tested on, including some methods specialized for the
relevant input domains.

Although the experiments reported here are restricted to learning a
Mahalanobis distance, the formulation we obtain 
allows for nonlinear similarity measures, as long as computing the
gradient of the objective in the algorithm is feasible. Furthermore,
our formulation naturally handles user-defined classification loss matrix, and not
just the vanilla zero-one loss.


\end{comment}







==> Chapters/Chapter09.tex <==
%************************************************
\chapter{Discriminative Group Equivariant Networks}\label{ch:gcnnintro}
%************************************************

\begin{aside}{Outline}
	In this part of the thesis we turn our attention to representational issues that were discussed in chapter \ref{ch:thesisintro}. In particular, in this review chapter,  we briefly motivate and discuss a recent research effort on discriminative representation learning, dubbed as \textbf{group equivariant neural networks}. Equivariance to symmetry transformations is explicitly encoded in the architecture in such networks; a classical convolutional neural network being one of the simplest examples. Indeed, a classical CNN is equivariant to translational symmetries in the input, also giving rise to its special topographic structure. We also argue that equivariance to appropriate symmetry transformations affords a strong inductive bias, and provides a rational design precept for the design of convolutional neural networks appropriate in different domains. 
\end{aside}

After a somewhat protracted slumber of more than a decade and a half, neural network based approaches, rechristened as \emph{deep learning}, made a remarkable comeback into the machine learning mainstream around 2006 \cite{HintonDBN, HintonScience, BengioGreedy}. Conceptually, it had been clear, and arguable with some force, albeit without direct theoretical backing, that architectures with many layers of non-linearities could represent \emph{highly-varying functions} \cite{LeCunAI} more efficiently. It was hypothesized that deeper networks could disentangle factors that explained the data better, affording compact, distributed representations \cite{HintonRumelhart} as compared to shallow architectures. However, it was not clear how to train deep architectures\footnote{A remarkable exception being Convolutional Neural Networks (CNNs) \cite{LeCun1989,LeCun1998}} till the influential works of Hinton \emph{et al.} \cite{HintonDBN, HintonScience}\footnote{The reader is pointed to \cite{SchmidhuberNN} for an exhaustive review and proper credit assignment}. These works led to a research program in the following years that was largely focused on unsupervised representation learning for preprocessing a downstream supervised task. This usually involved greedy, layer-wise pre-training of deep auto-encoders, deep generative models and the likes, and then fine-tuning them for a supervised task by using labels. One cartoon motivation for this program could be summarized as follows: feature representations that are good for modeling the data distribution $P(X)$, should also be good representations for the conditional distribution $P(Y|X)$. Unsupervised pre-training could be seen as attempting to model $P(X)$ better. A good review of approaches that fit under this general philosophy can be found in this (somewhat dated) monograph by Bengio \cite{BengioFNT}.

\vspace{2mm}
\noindent
Although the above program started to make deep learning competitive with more traditional approaches, the field could be said to have really taken off only in 2012 with the spectacular successes of CNNs on (then considered) difficult benchmark tasks \cite{Krizhevsky2012, MultiColumn}, also decidedly marking a shift in deep learning research from unsupervised representation learning to fully supervised discriminative representation learning\footnote{This is not to downplay the contributions made in the context of implicit density models \cite{GoodfellowGAN, Shakir} and progress in unsupervised learning since 2012}. Since then, such methods have come to dominate the machine learning landscape, with rapid advances in computer vision, speech recognition, natural language processing, drug discovery to name a few. The reasons for the dazzling successes of deep learning methods across a wide range of tasks are still not very well understood, and reviewing attempts would be beyond the scope of this chapter. However, one of the key principles that makes deep learning work in some domains is that of parameter (or weight) sharing. In particular, parameter sharing seems to help when it exploits the right symmetries and invariances pertaining to the problem at hand, thus providing a useful inductive bias. 

\vspace{2mm}
\noindent
In the next section we illustrate this in the context of CNNs and then also building some background for reviewing prior work on group equivariant CNNs.

\section{Classical CNNs, Translational Equivariance and Invariance}\label{sec:classicalCNN}

Before we talk about classical CNNs, it is perhaps instructive to define equivariance and invariance. We illustrate these (more general, mathematical) concepts in the context of concrete computer vision problems. First, consider the problem of image classification: Suppose we are working with images with 3 (RGB) channels, then an image could be seen as a function $f: \mathbb{Z}^2 \to \mathbb{R}^3$. Let us denote the space of functions $f: \mathbb{Z}^2 \to \mathbb{R}^3$ as $L_{\mathbb{R}^3}(\mathbb{Z}^2)$. Then, we can write the image classification problem as the map $L_{\mathbb{R}^3}(\mathbb{Z}^2) \to \{1, \dots, c \}$, where $c$ is the number of classes. One important symmetry inherent in the problem of image recognition is that of translation invariance. This is illustrated in figure \ref{fig:TransInv} (we would like the output of our system to remain unchanged if the image is translated). On the other hand, if we consider the problem of image segmentation such that the object of interest is assigned value 1, and rest of the image is assigned value 0 i.e. the map $L_{\mathbb{R}^3}(\mathbb{Z}^2) \to L_{\{0,1\}}(\mathbb{Z}^2)$, as illustrated in figure \ref{fig:TransEq}, we say that image segmentation is translation equivariant.

\begin{figure*}[!tb]
	\centering
	\begin{center}
		\includepic{.4}{./Chapters/Chapter09/cat.jpg}
	\end{center}
	\caption{Image recognition is translation invariant, the output of the learning system should not change if the input is translated by some amount $t$. Image is from ImageNet}
	\label{fig:TransInv} 
\end{figure*} 

\vspace{2mm}
\noindent
With these examples, we now define equivariance and invariance as follows:

\begin{aside}{Invariance, Equivariance and Covariance of $f(\cdot)$ w.r.t transformation $T_g(\cdot)$}
\begin{enumerate}
	\item[-] \textbf{Invariance: } $f(T_g(\cdot)) = f(\cdot)$
	\item[-] \textbf{Equivariance:} $f(T_g(\cdot)) = T_g(f(\cdot))$
	\item[-] \textbf{Covariance:} $f(T_g(\cdot)) = T_g^{'}(f(\cdot))$
\end{enumerate}
\end{aside}

\noindent
Where $T_g^{'}(\cdot)$ is a function of $T_g(\cdot)$. Thus covariance is a more general concept than equivariance (although both are often used interchangeably), which in turn is more general than invariance.

\begin{figure*}[!htb]
	\centering
	\begin{center}
		\includepic{.4}{./Chapters/Chapter09/catseg.jpg}
	\end{center}
	\caption{Image segmentation is translation equivariant}
	\label{fig:TransEq} 
\end{figure*}

\vspace{2mm}
\noindent
Having defined these terms, we return to talking about CNNs, our original motivation. CNNs were proposed in the context of image recognition, and as discussed, an important symmetry inherent in image recognition is that of translation invariance. While there might be many (and some not well understood) reasons for the success of CNNs, one important and well understood reason is that CNNs are inherently translational equivariant in the internal layers (modulo pooling and edge effects), and overall translation invariant. Translation equivariance is inbuilt in the architecture of a CNN, lending to it a somewhat unique topographic structure. To see this, let us consider the nuts and bolts of a $L+1$ layer CNN, for simplicity of exposition assume that we have only one channel. In a CNN neurons are arranged as a rectangular grid, thus the output of layer $\ell$ can be regarded as a function $f^{\ell}: \mathbb{Z}^2 \to \mathbb{R}$. The activations of layer $f^{\ell}$ are computed by taking the cross-correlation of the activations of the previous layer with a small learnable filter $h^{\ell}$ and then applying a suitable point-wise non-linearity on the output. 

\begin{equation}\label{eq:CNNcrosscorr}
(h^{\ell} \star f^{\ell - 1})(x) = \sum_{y} h^{\ell}(y-x) f^{\ell-1}(y) \qquad \qquad f^{\ell}(x) = \max\{0, (h^{\ell} \star f^{\ell - 1})(x)\}
\end{equation}

\noindent
To see why the above is translation equivariant, consider that we translate the feature map $f^{\ell-1}$ by an integer amount $t$ i.e. $f^{\ell-1} \mapsto T_t f^{\ell-1}$. Then, we have:

\begin{align}
	(h^{\ell} \star T_t f^{\ell - 1})(x) =& \sum_y f^{\ell-1}(y - t) h^{\ell}(y-x) \\
	=& \sum_y f^{\ell-1}(y) h^{\ell}(y - (x - t)) \\
	=& T_t (h^{\ell} \star f^{\ell-1}) (x)
\end{align}

\noindent
Thus showing that translating a feature map and then doing cross-correlation is the same as correlation followed by a translation. Ignoring pooling and edge effects; by induction, it is immediate that a CNN is translation equivariant upto layer $L$. The final layer $L+1$ is usually a softmax or classification layer, which now makes the CNN to be overall translation invariant. 

\vspace{2mm}
\noindent
Some of the take-home messages of the above discussion are: 
\begin{enumerate}
	\item[1] Translational symmetry is crucial in 2-D visual recognition, indeed, the output of a visual recognition system should approximately be invariant to shifts in the input. 
	\item[2] The CNN architecture explicitly enforces equivariance to translations by its special convolutional structure, causing each layer to preserve translational symmetry i.e. if the input is shifted by an amount $t$, ignoring pooling and edge effects, each feature map translates by the same amount. 
	\item[3] Exploiting translational symmetry is reflected in a drastic reduction in the number of parameters in a CNN as compared to a fully-connected feed-forward network when operating on images, since the same filter is applied across different image locations. 
\end{enumerate}

\noindent
In short, in the context of visual recognition, a classical CNN architecture exploits an important symmetry pertaining to the task i.e translational symmetry. Thus it could be seen as injecting an \emph{inductive bias} useful for the task at hand via its convolutional structure, thus aiding generalization. We refer the reader to experiments reported by Lenc and Vedaldi \cite{LencVedaldi} for some empirical evidence that equivariance in the image recognition context might indeed be a useful inductive bias. Note that the CNN structure obviates augmenting the data that involves supplying the network translated copies of the input during training. This is a theme we will return to later in this chapter. 

\vspace{2mm}
\noindent
Based on the above discussion, one might be naturally inclined to consider the following:

\begin{enumerate}\label{sec:pointsforGCNN}
	\item[1] Equivariance to translational symmetries in the context of image recognition seems like a conceptually sweet and rational design precept. It is perhaps also one of the main reasons (in view of the dissertation author) for the tremendous success of CNNs. Taking a cue from this, a natural question to ask would be: how to incorporate more symmetries useful for visual recognition in a planar CNN in a principled manner?
	\item[2] Enthused by the success of CNNs, there has been considerable effort to extend the idea to other domains, such as graphs, point-clouds, sets, manifolds \cite{pmlr-v48-niepert16,Duvenaud:2015:CNG:2969442.2969488, NIPS2016_6081,Masci:2015:GCN:2919341.2920992, DBLP:conf/cvpr/MontiBMRSB17, DBLP:journals/spm/BronsteinBLSV17} and so on. Thus, more generally than the point above: What is the natural way to generalize CNNs to such domains?
\end{enumerate}

\noindent
To motivate, we consider an example similar in spirit to that presented earlier. In particular, we consider the problem of 3-D shape classification. In this case, again assuming three channels marking the RGB values, each shape could be seen as a function $f: \mathbb{R}^3 \to \mathbb{R}^3$, and the classification problem is the map $L^2(\mathbb{R}^3, \mathbb{R}^3) \to \{1, \dots, c\}$. As illustrated in figure \ref{fig:RotInv} , 3-D shape classification is rotation invariant \footnote{We would infact want it to be invariant to rigid body motions, but we skip this for ease of exposition}. 

\begin{figure*}[!htb]
	\centering
	\begin{center}
		\includepic{.4}{./Chapters/Chapter09/ShapeNet.jpg}
	\end{center}
	\caption{Classification of 3-D shapes is rotation invariant (image from ShapeNet)}
	\label{fig:RotInv} 
\end{figure*}

\noindent
To solve the 3-D shape classification task in the same spirit as classical CNNs solve visual recognition, we would like to construct a network that is equivariant to 3-D rotational symmetries and overall invariant to them. That is, in the spirit of classical CNNs, we would like the network to be such that the activations at each layer in the network transform in a controlled way i.e. as a function of the transformation of the input. 

\vspace{2mm}
\noindent
From these two examples we might already get a sense of the nuts and bolts that we need to focus on to bring about a generalization of classical CNNs. In particular, there seem to be three things that seem essential to do so: The nature of the input space, the transformations of interest, and the transformations induced in the activations of each layer of some hypothetical neural network. In particular, when the input is subject to a transformation of interest, we want the activations to change as a function of the transformation on the input. In a classical CNN, the input space, denoted $X$ is the integer grid $\mathbb{Z}^2$. The transformations of interest are translations of the input. Let us denote the set of translations by $G$, it is clear that $G = \mathbb{Z}^2$. Next, when the input is translated by amount $t$, the activations in each layer (ignoring pooling and edge effects) also translate by the same amount. Note that if $G$ were instead a set of 3D rotations, then the whole enterprise wouldn't make sense. Indeed, there is a clear interplay between the transformations of interest and the input--it must be a symmetry of the input, that is, a transformation that leaves the input invariant. 

\vspace{2mm}
\noindent
What we are trying to get at by the above colloquial talk is that the set of transformations form a group $G$, in the algebraic sense of the word. The input set $X$ forms a $G$-space of the group $G$, while the activations at each layer transform as a function of the representation (again used in the algebraic sense of the word) of the transformation that the input is subjected to. It is this observation that lies at the heart of generalizing CNNs to a wide range of domains, and has been pioneered by the work of Cohen \emph{et al.} in a series of papers starting with \cite{Cohen2016}. This approach to generalizing CNNs, dubbed Group Equivariant Convolutional Neural Networks (GCNNs), following work by Cohen \emph{et al.} has lead to a somewhat burgeoning literature (see for instance \cite{Dieleman:2016:ECS:3045390.3045590, pmlr-v80-kondor18a, CohenSpherical18, Zaheer2017, Poczos2017, Cohen2017, NbodyArxiv18, ThomasTensor18, Boomsma2017, EstevesPo, Esteves, Worrall2016, Marcos2017, Jacobsen2017, Worrall2017, Cohen2018a, Cohen2018b, CohenSE3}). The purpose of this chapter is not to give an exhaustive overview of most recent work, but rather review the salient features in an intuitive manner so as to make the motivation of group equivariant representation learning and its connection to convolutions clear. 

\vspace{2mm}
\noindent
Next, we introduce some definitions in order to proceed and formalize some of the informal discussions made above. 



\section{Elementary Definitions}

First, let us define groups:

\begin{aside}{Groups}
	A group is a set $\mathcal{G}$ endowed with an internal composition operation, that we refer to as group multiplication and denote by $\ast$. $\forall a, b \in \mathcal{G}$ we have $\ast: \mathcal{G} \times \mathcal{G} \to \mathcal{G}$
	such that the following conditions are satisfied: 
	\begin{enumerate}
		\item \textbf{Associativity:} $\forall a, b, c \in \mathcal{G}$, $(a \ast b) \ast c = a \ast (b \ast c)$
		\item \textbf{Existence of identity:} $\exists e \in \mathcal{G}$ such that $a \ast e = a = e \ast a$, moreover the left and right identities are equal and unique.
		\item \textbf{Existence of inverses:} $\forall a \in \mathcal{G}$, $\exists a' \in \mathcal{G}$ such that $a \ast a' = e = a' \ast a$, moreover the left and right inverses are equal and unique.
	\end{enumerate}
\end{aside}

\begin{aside}{Group Actions}
 	For a set $X$ and a group $\mathcal{G}$, a group action is an associative map $\phi: \mathcal{G} \times X \to X$, such that $\phi(e,x) = x$, $\forall x \in X$
\end{aside}

\section{Planar CNNs as Group Equivariant Neural Networks}
Recall that the crucial property of CNNs is that if the input $f^0$ is subject to a transformation (in this case a translation) denoted $T_t$ i.e. $f^0 \mapsto T_t^0[f^0]$, then at layer $\ell$, we see the same effect $f^{\ell} \mapsto T_t^{\ell}[f^{\ell}]$. In particular, here, $T_tT_t^{\ell}$

Classical CNNs can be seen as simplest examples of a group-equivariant CNN, where the group in question is the group of integer translations $\mathbb{Z}^2$.

Then show the original Cohen welling thing for discrete groups, and also show that it already has all the ingrediants of more general networks. 

Then there are continuous networks, in such networks it is natural to proceed to Fourier space. Have a discussion about this. Then introduce the general group conv formula over compact groups, state the theorem, and then also point to the Fourier picture. Say in words what it means. 

This really establishes that in order to obtain generalized cnns, you have to really work with generalized convolution. 

but the success of CNNs does tell us something important. Exploit the right thng for the problem and you have a strong inductive bias. They also serve as a regularizer. Not well understood, but there are two things that are clear. Exploit translation symmetries . 

The unsupervised resurgence was attributed to many things. But in many cases it was not clear what was happening. The shift then happened to fully discriminative methods. Since then, they have been used all over the place. Now, how do you have the right representation? A representation is useful if?
That leads us to objects of our interest. Augment data in CNNs, what if these symmetries are inbuilt in them? 

\begin{definition}[Group Convolution]
Let $X$ denote a $G$-space, and let $f, g: X \to \mathbb{C}$ be functions defined on the $G$-space. The convolution of $f$ and $g$ is a function on $G$, that we call Group-convolution or simply $G$-convolution, is defined as:
\begin{equation}
f \ast g =  \int_X f(R^{-1} \cdot x) g(x) dx
\end{equation}	
\end{definition}

\begin{aside}{All equivariant networks are Group CNNs}
\begin{theorem}[Kondor and Trivedi \cite{pmlr-v80-kondor18a}]
A neural network connecting layers of the form $L^2(X_i, \mathbb{C}^{n_i})$ for a sequence of $G$-spaces $X_i$ is G-equivariant if and only if it is a composition of $G$-convolutions on the $X_i$ spaces and nonlinearities applied to $\mathbb{C}^{n_i}$
\end{theorem}
\end{aside}

For a while all work was on image based CNNs. But what about other domains? How do equivariance and multiscale structure interact?

\textcolor{red}{this is a placeholder chapter -- add new tex and keep some of the survey here}

In the past few years rapid advances in computer vision, speech recognition, natural language processing etc., have been afforded by deep learning. 

 The case of CNNs in the image recognition domain, where the output should be invariant to translations of the input, is particularly instructive: 1) The convolution operation preserves the topographic structure of the original image, making it equivariant to translation. That is, if the input image is translated, then the activations in higher layers change in a controllable way. 2) As we go deeper in the network each neuron is responsible for more of the input than neurons in earlier layers, allowing the network to capture structure at multiple scales.

Both of these properties are a direct consequence of the convolution formula: convolution is equivariant to actions of the translation group on the input (an image). More recent work has tried to design image based CNNs that try to exploit more symmetries, such as warps, rotations and flips, allowing greater parameter sharing. Even more recent work has focused on extending CNNs to more general input structures such as graphs. While a number of different architectures have been proposed that are inspired by CNNs, it is not clear what the right mathematical notion of convolution in such cases is. This is not just a case of a technical detail, as it has a bearing on how it relates to equivariance, or if the right symmetries of the problem are exploited. 

In this thesis we propose to undertake a systematic study of the behavior of feedforward networks under transformations. As a first step we show that infact convolution is a necessary and sufficient condition for equivariance in feed-forward networks, not just in image recognition, but with respect to the action of any compact group acting on a sequence of homogeneous spaces. Next, the case is made that in many applications where the input has a non-trivial combinatorial structure, convolution alone is not rich enough to capture structure. We introduce a generalization called steerable convolution and also show that it is a necessary and sufficient condition for the corresponding notion of equivariance.

The import of these two results is not merely theoretical, it naturally allows for constructing general equivariant compositional neural networks. We propose two applications: One to graphs, where each elementary part corresponds to a vertex and the network itself corresponds to a hierarchy of parts. The activation of each neuron in this network co-varies with a permutation of the input. The second application is to design a fully Fourier space $SO(3)$-equivariant CNN for data that lives on a sphere. The latter also introduces a formalism that applies more generally i.e. for the design of Fourer space neural networks that are equivariant to the action of any continuous compact group.

In the next section, we first discuss some related literature on equivariant and invariant representation learning, with a focus on steerability.





%*****************************************

The study of steerable filters originated in the context of low-level computer vision and image processing applications, such as edge detection, texture analysis, image compression etc \cite{FreemanAdelson1991}. In many such applications it is often needed to apply a filter with arbitrary orientation and to consider the response as a function of the orientation and phase. The idea in  \cite{FreemanAdelson1991} was to efficiently \emph{steer} filters at arbitrary orientations by taking an appropriate linear combination of a set of basis filters. \cite{Perona1995} and \cite{TeoHelOr1999} used steerability to approximate feature detectors tuned to particular orientations by convolving an image with basis filters and taking an interpolation between them. This was later used to design filter banks that detected features at multiple orientations efficiently \cite{Manduchi1998}. It is worth noting that to steer a fixed function with an arbitrary compact transformation, the approach of \cite{Perona1995} computes the optimal basis functions in the least squares sense. On the other hand, \cite{TeoHelOr1999} employ Lie group-theoretic methods. The function to be steered is first approximated by a linear combination of equivariant functions (basis functions) and then steered using them. A representative of one flavour of extensions to \cite{FreemanAdelson1991} and some of the work reviewed above is the steerable pyramid  \cite{Simocelli1992}, which was used to decompose an image linearly into scale and orientation subbands. Steerable pyramids were used in a number of applications; image denoising \cite{Portilla2003} and texture characterization \cite{Do2002} to name a couple.

Use of group theoretic methods for feature extraction and steerability has been around in the literature for a while, albeit appearing sparsely \cite{Lenz1989} \cite{Wood1996} \cite{Casey1998} \cite{Kondor2007} \cite{Kondor2008}. Amongst the first in the literature on the topic, \cite{Lenz1989} tries to motivate steerability (without explicitly using the term) by observing that set of input signals are not structureless but can be divided into different subspaces in such a way that signals in a particular subspace are connected to each other by means of a group transformation. It is assumed that the signal space is symmetrical or that the subspaces are invariant under the group operation. A similar approach was motivated by \cite{KoVanDoorn1990} with the goal of giving a principled taxonomy of linear spatial receptive field structures. \cite{Michaelis1995} extend the methodology of \cite{FreemanAdelson1991} and \cite{Simocelli1992} (which steered filters by Fourier decompositions) and justify steerability based on Lie group theory, although they only consider Abelian Lie groups. Their approach is extended to all Lie groups by \cite{TeoHelOr1999}, and further generalized by \cite{Krajsek2007}.

The papers referenced thus far are about steerable filters and their motivation via group representation theory. These kernels are not learned and only apply to low level vision applications. In high level applications we are interested in the more general case of high dimensional \emph{representations} that are steerable as well as learnable. There is a large body of literature, particularly in computer vision, on learning invariant representations (one of the more famous examples of which was SIFT \cite{Lowe04}). However, in high level applications it is not desirable to have the intermediate representations (as in deep neural networks) to be fully invariant. Rather, it is far more useful to have representations that preserve the relative pose of local features motivating equivariant and steerable representations. Representations that transform in a controlled manner under transformations of the input are equivariant representations. We first review some literature on learning equivariant representations and then review more recent work that uses representation theory, as in the case of steerable filters, providing a natural framework for steerability.

One of the earliest works on constructing equivariant representations goes back to \cite{Hinton1981} which considered assigning canoncical frames of references to object parts. This was extended further in \cite{HintonWang2011} where instead of a scalar feature detector, features were thought of as organized in groups (\emph{capsules}) which include both the pattern detector and a set of pose parameters that specify the pattern. \cite{Tieleman2014} extends this framework further by explicitly transforming parts by mappings learned by the network. Some other work on equivariant representations includes the transformation equivariant restricted Boltzmann machine \cite{KivinenWilliams2011}, equivariant kernels and filtering \cite{Reisert2008}, \cite{Skibbe2013}. The M-theory of \cite{Anselmi2014} also studies invariant and equivariant representations. They construct features that are invariant to a symmetry group by using averaged statistics of dot products with the group orbits. A major drawback of the methods reviewed in this paragraph is that none of them are discriminatively trained.

In order to discriminatively learn representations that are invariant, or more generally, equivariant with respect to image transformations; there is recent interest in the context of convolutional neural networks \cite{Gens2014} \cite{CohenWell2015} \cite{Dieleman2016} \cite{Kanazawa2014} \cite{Cohen2016} \cite{Cohen2017} \cite{Marcos2017} \cite{Jacobsen2017} \cite{Worrall2017}. The authors in \cite{Gens2014} propose an CNN that gives feature maps over arbitrary symmetry groups, giving an approximately equivariant architecture. The work of \cite{Dieleman2016} constructs a network that is experimentally shown to be equivariant to rotation and was applied to vision problems that have cyclic symmetry. \cite{CohenWell2015} use group representation theory to study the equivariance properties of CNNs and then propose a more general CNN that exploits larger groups of symmetries by using Group-convolutions. Furthermore, they show that various modules used in modern CNNs such as pooling, pointwise non-linearities, batch normalization, residual blocks are equivariant as well. \cite{CohenWell2015} \cite{Gens2014} and other papers referenced above implicitly or explicitly use a very particular kind of representation called the regular representation. \cite{Cohen2017} give a more general theory of steerable representations that decouples the size of the group from learning equivariant representations. This theoretical treatment puts in sharp relief a type system in which any steerable representation is a composition of elementary feature types represented by capsules (reminiscent of \cite{HintonWang2011}). Thus, methods that use the regular representation are restricted to a particular kind of capsule. Our work builds on top of \cite{Cohen2016} \cite{Cohen2017} to build steerable representations for combinatorial data as well as further giving theoretical justification.

It is also worth mentioning that scattering networks \cite{Mallat2012} \cite{Bruna2013}\cite{Sifre2013}\cite{Oyallon2015} also use the regular representation. Scattering networks use wavelet convolutions, non-linearities and averaging to give rise to stable invariants\cite{Mallat2012} \cite{Bruna2013}. The work of \cite{Sifre2013}\cite{Oyallon2015} extends this notion to convolutions on the larger group of translations, rotations and scaling. One major drawback of scattering networks is, that has limited their applicability, is that they are not discriminatively trained.

In most of the work reviewed above, the inputs are assumed to live in $\mathbb{Z}^2$. There is a lot of recent interest to extend convolutional neural networks to combinatorial data, in particular graphs. The primary challenge here is to first define a precise notion of convolution, as well as construct representations that are steerable. Some approaches to CNNs on graphs essentially try to mimic image-based CNNs by defining a convolution like operator that acts on locally connected regions of the input. For example, the approach of \cite{Niepert2016} is predicated on the observation that feature computation in a regular CNN can be seen as traversing a node sequence and doing some local computation centered at each node. Thus, in their approach defining the CNN for a graph boils down to first determining the sequence of nodes to traverse, and then computing features using neighborhood graphs during the traversal. However, for arbitrary graphs, the vertex ordering is not unique and it is also not clear if this neighborhood operator corresponds to a mathematically precise notion of convolution. Yet another set of approaches fall into the so-called label propagation framework \cite{Duvenaud2015} \cite{Li2016} \cite{Riley2017} \cite{Kearns2016}. The essence of this approach is the following: At level $\ell = 0$ each vertex $v$ is initialized with its base label $\phi_0(v)$. At levels $\ell = 1 \dots L$, the label for each vertex $v$ is recalculated by considering all the previous labels for each of its neighbors. The representation for the graph $\phi(G)$ is then computed by aggregating the top level labels for all vertices. Repeated aggregation of information and passing it through a non-linear activation function resembles convolutional neural networks and this is emphasized by the authors. However there is a notable difference: In regular convolutional networks the intermediate representations are covariant with image transformations, while most label propagation schemes are only invariant. Our work tries to precisely define convolution on combinatorial data, especially graphs and constructing representations that are steerable.

Lastly, in the context of CNNs on graphs, a passing reference must be made to a growing body of (only superficially related) work that tries to extend CNNs to non-regular domains i.e. topologies that differ from a 2D grid structure \cite{Bruna2014} \cite{Henaff2015} \cite{Defferrard2016}. These approaches assume one global graph structure and work with functions defined on graphs, implying a correspondence between vertices across inputs. Such approaches are not applicable where every input can be an arbitrary graph.

%*****************************************
%*****************************************
%*****************************************
%*****************************************

